Self-Supervised Masked Mesh Learning for Unsupervised Anomaly Detection on 3D Cortical Surfaces

Unsupervised anomaly detection in brain imaging is challenging. In this paper, we propose self-supervised masked mesh learning for unsupervised anomaly detection on 3D cortical surfaces. Our framework leverages the intrinsic geometry of the cortical surface to learn a self-supervised representation that captures the underlying structure of the brain. We introduce a masked mesh convolutional neural network (MMN) that learns to predict masked regions of the cortical surface. By training the MMN on a large dataset of healthy subjects, we learn a representation that captures the normal variation in the cortical surface. We then use this representation to detect anomalies in unseen individuals by calculating anomaly scores based on the reconstruction error of the MMN. We evaluated our framework by training on population-scale dataset UKB and HCP-Aging and testing on two datasets of Alzheimer's disease patients ADNI and OASIS3. Our results show that our framework can detect anomalies in cortical thickness, cortical volume, and cortical sulcus characteristics, which are known to be biomarkers of Alzheimer's disease. Our proposed framework provides a promising approach for unsupervised anomaly detection based on normative variation of cortical features.

==> 6-limitations.tex <==
\section{Limitations}\label{sec:limitations}

Despite the promising results of our self-supervised masked mesh learning framework for unsupervised anomaly detection in 3D cortical surfaces, several limitations must be acknowledged. One key limitation is that the performance of our framework requires extensive hyperparameter tuning for different datasets, which can restrict its generalizability across varied populations and imaging conditions \cite{yang2020hyperparameter}. This tuning process can be time-consuming and may not always achieve optimal results for every dataset, potentially impacting the framework's ability to perform consistently across diverse scenarios. To address this limitation, future research could focus on training the model on more diverse datasets. By incorporating a wider range of data sources, including variations in imaging protocols, populations, we can potentially enhance the model's robustness and improve its ability to generalize. Previous studies suggest that training on a broader array of data can lead to greater generalizability, especially in applications related to brain aging and other dynamic neurological processes \cite{leonardsen2023genetic}. Expanding the diversity of the data set could help the model better adapt to different anatomical and pathological variations, thus improving its applicability and precision in a wider range of clinical settings. Additionally, exploring techniques such as domain adaptation and transfer learning could further mitigate the limitations related to dataset-specific tuning. These approaches might enable the model to leverage knowledge from one dataset to improve performance on another, thus enhancing its generalization and utility. By addressing these limitations and broadening the scope of training data, our framework has the potential to become a more versatile and widely applicable tool to detect cortical anomalies in various neurological and psychiatric conditions.

Training and fine-tuning the model for unsupervised anomaly detection in 3D cortical surfaces require considerable computational power due to the complex nature of the data and the intensive calculations involved in processing and analyzing large-scale brain imaging datasets. Our reliance on reconstruction error as the primary metric for anomaly detection may present limitations, as it might not fully capture subtle or complex anomalies in the cortical surfaces \cite{darayi2022computational,schwartz2023evolution}. Reconstruction error measures the discrepancy between the original and reconstructed data, which is useful for identifying obvious deviations from the norm. However, subtle or intricate anomalies, which might be indicative of early or nuanced pathological changes, may not significantly affect the overall reconstruction error or anomalies that are spread over space \cite{lamballais2020cortical,demirci2023systematic}. This limitation suggests that, while the reconstruction error is a valuable tool, it may not be sufficient on its own for a comprehensive detection of all types of anomalies. To address this issue, it is crucial to integrate additional metrics and analytical approaches that can complement the reconstruction error. Metrics such as feature-based similarity measures, statistical outlier detection, or domain-specific anomaly scores could help identify subtle or complex anomalies in nature \cite{tschuchnig2022anomaly}.

==> f_oneway-adni.tex <==
\begin{table*}[t!]
    \caption{Results of one-way ANOVA analysis on the ADNI dataset. * indicates $p < 0.05$, ** indicates $p < 0.01$.}
    \resizebox{\textwidth}{!}{%

        \begin{tabular}{@{}ccc@{}}
            \toprule
                      & \textbf{Left Hemisphere}                          & \textbf{Right Hemisphere}  \\ \midrule\midrule
            Curvature & insula**, inferiorparietal*                       & insula**                   \\ \midrule
            Sulcus    & \begin{tabular}[c]{@{}c@{}}postcentral**, parahippocampal**, fusiform**\\ precentral**, middletemporal*, temporalpole*\\ superiorfrontal*\end{tabular}                         & postcentral*               \\ \midrule
            Thickness & \begin{tabular}[c]{@{}c@{}}entorhinal**, precentral**, transversetemporal**\\ parsopercularis**, parsorbitalis**, posteriorcingulate*\\ lateralorbitofrontal*, pericalcarine*, precuneus*\\ parstriangularis*, superiorfrontal*, superiorparietal*\\ middletemporal*, inferiorparietal*, lateraloccipital*\end{tabular}                         & \begin{tabular}[c]{@{}c@{}}precentral**, precuneus**, inferiorparietal*\\ caudalanteriorcingulate*\end{tabular}  \\ \midrule
            Volume    & entorhinal**, parsorbitalis**, parstriangularis** & entorhinal**, precentral** \\ \bottomrule
        \end{tabular}
    }
    \label{table:f_oneway-adni}
\end{table*}

==> f_oneway-oasis3.tex <==
\begin{table*}[t!]
    \caption{Results of one-way ANOVA analysis on the OASIS3 dataset. * indicates $p < 0.05$, ** indicates $p < 0.01$.}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}ccc@{}}
            \toprule
                      & \textbf{Left Hemisphere}  & \textbf{Right Hemisphere} \\ \midrule
            Curvature & -                         & -                         \\ \midrule
            Sulcus    & \begin{tabular}[c]{@{}c@{}}fusiform**, postcentral**, parahippocampal**\\ lateraloccipital*, entorhinal*, inferiortemporal*\\ isthmuscingulate*, lingual*, posteriorcingulate*\\ precentral*, transversetemporal*, insula*\\ inferiorparietal*, caudalanteriorcingulate*\end{tabular} & \begin{tabular}[c]{@{}c@{}}supramarginal**, fusiform**, paracentral**\\ inferiorparietal**, medialorbitofrontal**, \\ insula**, pericalcarine**\end{tabular} \\ \midrule
            Thickness & \begin{tabular}[c]{@{}c@{}}superiorfrontal**, precentral**, supramarginal**\\ caudalmiddlefrontal**, cuneus**, caudalanteriorcingulate**\\ transversetemporal**, bankssts**, parsopercularis**\\ superiorparietal**,  entorhinal**, precuneus**\\ lateraloccipital**, parsorbitalis**, insula**\\ pericalcarine**, superiortemporal**, postcentral*\\ rostralmiddlefrontal*, middletemporal*, posteriorcingulate\\ frontalpole*, rostralanteriorcingulate*\end{tabular} & \begin{tabular}[c]{@{}c@{}}precentral**, caudalmiddlefrontal**,\\ caudalanteriorcingulate**, cuneus**, superiorfrontal**\\ lateraloccipital**, inferiorparietal**, parsopercularis**\\ precuneus**, entorhinal**, posteriorcingulate**\\ superiorparietal**, pericalcarine**, supramarginal*\\ paracentral*, parsorbitalis*\end{tabular} \\ \midrule
            Volume    & \begin{tabular}[c]{@{}c@{}}rostralmiddlefrontal**, lateralorbitofrontal**, insula**\\ medialorbitofrontal**, lingual**, superiorfrontal**\\ parstriangularis**, transversetemporal**, fusiform**\\ middletemporal**, parsopercularis**, posteriorcingulate**\\ caudalanteriorcingulate**, frontalpole*, paracentral*\\ bankssts*, temporalpole*, caudalmiddlefrontal*\\ precentral*, postcentral*,  rostralanteriorcingulate*\end{tabular} & \begin{tabular}[c]{@{}c@{}}lateralorbitofrontal**, rostralmiddlefrontal**\\ medialorbitofrontal**, parstriangularis**\\ inferiorparietal**, caudalanteriorcingulate**\\ lingual**, parsopercularis**, middletemporal**\\ supramarginal*, pericalcarine*, temporalpole*\\ precentral*, superiorfrontal*\end{tabular} \\ \bottomrule
        \end{tabular}

    }
    \label{table:f_oneway-oasis3}
\end{table*}

==> result-1way_anova_adni.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.9\textwidth]{figure2-result-1way_anova-eta-adni.pdf}
    \caption{Unsupervised anomaly detection result in Adni dataset.}
    \label{fig:result_1way_anova_eta_adni}
\end{figure*}

==> result-1way_anova_oasis3.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.9\textwidth]{figure2-result-1way_anova-eta-oasis3.pdf}
    \caption{Unsupervised anomaly detection result in OASIS3 dataset.}
    \label{fig:result_1way_anova_eta_oasis3}
\end{figure*}
